Measuring Emergent Capabilities of LLMs for Software Engineering: How Far Are We?

The adoption of Large Language Models (LLMs) across multiple contexts has sparked interest in understanding how scaling model size might lead to behavioral changes, as LLMs can exhibit behaviors not observed in their smaller counterparts. Understanding these emergent capabilities is essential for advancing LLM development and improving their interpretability across diverse tasks. However, whether LLMs exhibit true emergence in the context of Software Engineering remains an unexplored topic, as most research has focused on NLP tasks. In this paper, we investigate the emergence of capabilities in the context of SE. We propose a model-agnostic pipeline for evaluating this phenomenon across three SE tasks: bug fixing, code translation, and commit message generation. More precisely, for each task, we present a case study instantiating our pipeline to analyze the emergence of capabilities in CodeGen1-multi across four scales ranging from 350M to 16.1B parameters. Our findings do not not provide evidence to support the idea of emergent capabilities resulting from scaling the model size in the selected set of tasks. We hope our results can pave the way to a more nuanced understanding of emergent capabilities of LLMs within the SE domain, guiding future research to focus on task-specific evaluations and the identification of alternative factors contributing to this phenomenon. Our work underscores the importance of task diversity in examining model behaviors and highlights potential limitations in transferring prior understandings of and approaches to emergence from NLP to Software Engineering.

==> bk/Zdump.tex <==
% dummy file containing unused sentences and paragraphs.


%%% FROM `introduction.tex`: %%%

%In fact, most LLMs are not organized as a family of models varying by scale, but monolithic \cite{touvron2023llama}.

%and attempts to falsify claims of emergent capabilities work by demonstrating the smooth relationship between model scale and performance \cite{schaeffer2023emergent,lu2023emergent}.


% Whether Large Language Models (LLMs) can exhibit capabilities which appear unpredictably upon scaling them large enough is both an alarming and powerful prospect. This phenomenon has the potential to both unlock new planes of improvement on tasks, as well as unprecedented harmful capabilities \ALEJO{do you have references to support this claim? what are those harmful capabilities?}. Therefore, establishing a reliable methodology of investigating emergent capabilities is crucial to responsible and continued development of LLMs \ALEJO{it is not clear here why do we need to study the problem, this sentence should be a conclusion of the problem in the next paragraph}. While much research has been conducted on LLM's emergent capabilities in the domain of natural language processing (NLP), most of the discourse until now has focused primarily on assessing whether researchers have correctly demonstrated the phenomenon as a property of models, or if it is the case that researchers have merely induced these findings by choice of metric \cite{schaeffer2023emergent}, or if emergent capabilities are better explained through its prowess in the more generic ability to learn from examples in its input, or as a description of capabilities which do not strongly require reasoning \cite{lu2023emergent} \ALEJO{if the idea here is to talk about studies in NLP regarding capabilities, you should only mention the main takeaways. listing sources here is inconvenient, they should be included in the related work instead}.

%%% Our study seeks to investigate emergent capabilities exclusively in the context of software engineering tasks, a novelty in the discourse. Software engineering tasks and the corresponding capabilities required of LLMs to solve them differ notably from those required to solve the natural language processing tasks which have hitherto been the primary focus of study in the field of emergent capabilities.

%%%Furthermore, our study analyzes capabilities relevant to the field of software engineering, such as automatic bug fixing and commit message generation, data about which would be relevant to LLMs targeting this domain designed to assist programmers in this field.

%%% Although state-of-the-art LLMs have proven increasingly capable on a wide variety of tasks \cite{brown2020language} \cite{doi:10.1098/rsta.2023.0254}, especially in the domain of Natural Language Processing, many models and model architectures are trained on and adapted to the realm of software engineering: T5 \cite{raffel2023exploring} spawned CodeT5 \cite{wang2021codet5}, BERT\cite{devlin2019bert} spawned CodeBERT \cite{feng2020codebert}, and LLaMA \cite{touvron2023llama} spawned Code Llama \cite{rozière2024code}. In other words, there is widespread precedent for developing LLMs specific to the domain of software engineering. Likewise, though research on emergence in LLMs hitherto has been focused on NLP tasks, virtually none has been directed predominately towards the field of software engineering.

% \Fakesubsection{Problem}

%%% The notion of emergent capabilities has long been a subject of inquiry in the field of machine learning. As early as 2020 and 2021, researchers were concerned about the negative side effects of increasing model scale, particularly with increasingly larger models adopting the explicit and implicit biases featured in their training sets, and their ability to mimic coherent human speech and articulation \cite{bender2021parrots}, based on concerns and research done into the various kinds of bias found in models such as BERT, GPT-2, and GPT-3 \cite{Guo_2021} \cite{hutchinson-etal-2020-social}.

% \ALEJO{a short definition of emergence should be in the previous paragraph. There are citations here without proper references. Again the idea here is not to describe the related work, but just to provide a glance of the overall picture. This paragraph should define the problem you aim to address in your research, which is not still clear.}
% Researchers have used the term \textit{emergence} to refer to capabilities which models acquired through training that they were not explicitly trained for, as in Nijkamp et al.'s \cite{nijkamp2023codegen} paper documenting the CodeGen family, where the term is used to describe the model's capability to synthesize programs from comment descriptions. \ALEJO{This is a separate idea and should be in a diferent paragraph} The rigorous study of emergent capabilities, however, was made most prominent with Wei et al., where emergent capabilities are framed not as capabilities acquired without explicit intentions, but as sharp, unpredictable jumps in performance \cite{wei2022emergent}. Their findings suggest that LLMs, through certain tasks and prompting methods, when scaled high enough (e.g. by training compute or parameter count), can unexpectedly and noticeably break a plateaued trend in performance. \ALEJO{When using adjectives try to use simpler words, as they are more suited for scientific writing.}

% However, various researchers contest the claim that these models exhibited emergent capabilities whatsoever. Shaeffer et al. \cite{schaeffer2023emergent} suggest the appearance of emergence is better explained by the metrics used to assess model performance, rather than as some property of the model itself; they implicate nonlinear and discontinuous metrics as a confounding factor in Wei et al.'s results. Other research by Lu et al. suggests what appears to be emergent capabilities are better explained as the results of in-context learning, that is, the model's ability to derive crucial information from the context it is prompted with and apply that knowledge to the task at hand \cite{lu2023emergent}.

% \ALEJO{What is the problem here? if you want to say the problem is the definition of emergence in the context of SE, you should mention it explicitly. }

% \Fakesubsection{Motivating Example}


% Suppose we want to develop an LLM to accomplish automatic bug repair, that is, transforming buggy code to fixed code. In the interest of iterative development, we start at a small model scale, and incrementally scale the model size, and we want to observe how the performance changes. Simply, one could calculate the proportion of the validation set tests the model passes exactly, and compare this proportion across the various model scales, and assess the results qualitatively, albeit somewhat imprecisely. What if we wanted to talk more precisely about the relationship between model scale growth and performance? When should we stop increasing model scale? How exactly should we assess performance? Can our models be used in other contexts? Can we be confident that the model does not degrade in other context, that is, ``improve'' in degenerate aspects? \ALEJO{List only the questions that you want to solve in your research, I dont think you are addressing all of them. }

% \ALEJO{Again, use simpler words, what is a "plateau" in this context? What is the main idea of this paragraph? there are many ideas mixed together. }
% The discussion of emergent capabilities for LLMs is central to answering these questions. If LLMs are capable of exhibiting emergent capabilities in certain circumstances, then we can augment our analysis of plateaus in model performance with the notion that, at a certain scale, the model may emergently escape that plateau, perhaps giving credence to the idea of adding more scale to the model without immediate, tangible performance increases. Furthermore, we need not restrict our inquiries to performance on the validation set: By introducing external datasets into our model assessment process, we can gauge the rate at which our models acquires these other skills, and if they do so at an emergent rate. \ALEJO{ You are implying that by using evaluation datasets we are able to measure the emergency of capabilities?} Conversely, we can evaluate our model on degenerate datasets, and evaluating how that score changes with scale. By having a firm foundation with which to consider emergent capabilities, our ability to interpret LLMs increases.

%%% \TODO{present small, very constrained example of how emergency of how it has been demonstrated previously}

%%% \TODO{\textbf{Hypothetical example} - we have a model, assert the model is bad at task X; we can observe the model can improve the performance when we escalate size; we conduct this study to understand emergence}

% \Fakesubsection{Proposed Solution}
% \ALEJO{The image that you introduce here, should be in the methodology section, the intro should only contain a short description of the overall solution. Still, it is not clear what is the solution since the problem is not defined correctly in the first place. }



